BEAGLE: Forensics of Deep Learning Backdoor Attack for Better Defense

Deep Learning backdoor attacks have a threat model similar to traditional cyber attacks. Attack forensics, a critical counter-measure for traditional cyber attacks, is hence of importance for defending model backdoor attacks. In this paper, we propose a novel model backdoor forensics technique. Given a few attack samples such as inputs with backdoor triggers, which may represent different types of backdoors, our technique automatically decomposes them to clean inputs and the corresponding triggers. It then clusters the triggers based on their properties to allow automatic attack categorization and summarization. Backdoor scanners can then be automatically synthesized to find other instances of the same type of backdoor in other models. Our evaluation on 2,532 pre-trained models, 10 popular attacks, and comparison with 9 baselines show that our technique is highly effective. The decomposed clean inputs and triggers closely resemble the ground truth. The synthesized scanners substantially outperform the vanilla versions of existing scanners that can hardly generalize to different kinds of attacks.

==> tables/ablation_transparency.tex <==
\begin{table}[h]
    \centering
    % \footnotesize
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    \caption{Ablation study of different transparency
    \siyuan{We show that 0.3 is generally a good transparency parameter which both achieve high visual quality and attack effectiveness.}
    }
    \label{tab:transparency}
    \begin{tabular}{cc|cccc|cccc}
        \toprule
        \multirow{2}{*}{\textbf{Backdoor}} & \multirow{2}{*}{\textbf{Alpha}} & \multicolumn{4}{c}{\textbf{Removal}} & \multicolumn{4}{c}{\textbf{Injection}} \\
        ~ & ~ & L1 & PSNR & SSIM & ACC & L1 & PSNR & SSIM & ASR \\
        \hline
        % Reflection
        \multirow{5}{*}{\textbf{Reflection}} & 0.1 & 0.226 & 20.59 & 0.81 & 1.0 & 0.335 & 17.25 & 0.73 & 0.14 \\
        ~ & 0.2 & 0.219 & 20.81 & 0.81 & 1.0 & 0.269 & 19.13 & 0.79 & 0.76 \\
        ~ & 0.3 & 0.215 & 20.96 & 0.81 & 1.0 & 0.194 & 21.62 & 0.85 & 0.95 \\
        ~ & 0.4 & 0.216 & 20.90 & 0.81 & 1.0 & 0.160 & 23.13 & 0.88 & 0.97 \\
        ~ & 0.5 & 0.254 & 19.24 & 0.75 & 1.0 & 0.267 & 18.55 & 0.77 & 0.98 \\
        \hline\hline
        % SIG
        \multirow{5}{*}{\textbf{SIG}} & 0.1 & 0.190 & 21.96 & 0.84 & 1.0 & 0.158 & 24.33 & 0.86 & 0.32 \\
        ~ & 0.2 & 0.191 & 21.88 & 0.84 & 1.0 & 0.077 & 27.86 & 0.96 & 0.87 \\
        ~ & 0.3 & 0.192 & 21.84 & 0.83 & 1.0 & 0.148 & 24.83 & 0.96 & 0.97 \\
        ~ & 0.4 & 0.201 & 21.50 & 0.82 & 1.0 & 0.184 & 22.72 & 0.94 & 0.99 \\
        ~ & 0.5 & 0.234 & 20.35 & 0.79 & 1.0 & 0.214 & 21.43 & 0.90 & 1.0 \\
        \hline\hline
        % Blend
        \multirow{5}{*}{\textbf{Blend}} & 0.1 & 0.193 & 21.93 & 0.84 & 1.0 & 0.116 & 26.43 & 0.84 & 0.97 \\
        ~ & 0.2 & 0.197 & 21.78 & 0.84 & 1.0 & 0.117 & 26.14 & 0.92 & 1.0 \\
        ~ & 0.3 & 0.203 & 21.52 & 0.83 & 1.0 & 0.155 & 24.06 & 0.90 & 1.0 \\
        ~ & 0.4 & 0.209 & 21.27 & 0.83 & 1.0 & 0.192 & 22.29 & 0.85 & 1.0 \\
        ~ & 0.5 & 0.216 & 21.00 & 0.81 & 1.0 & 0.243 & 20.25 & 0.75 & 1.0 \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/dataset_cleaning.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Dataset Cleaning}
    \label{tab:data_clean}
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
         \toprule
         \multicolumn{13}{c}{\color[HTML]{FE0000} \textbf{CIFAR-10 \& VGG-11}} \\
         \midrule
         \textbf{Attack} & \multicolumn{2}{c}{\textbf{ACC}} & \multicolumn{2}{c}{\textbf{FP}} & \multicolumn{2}{c}{\textbf{FN}} & \multicolumn{2}{c}{\textbf{FFR}} & \multicolumn{2}{c}{\textbf{FAR}} & \multicolumn{2}{c}{\textbf{Time (s)}} \\
         \midrule
         BadNets & 0.97 & 0.98 & 28 & 76 & 153 & 9 & 0.01 & 0.02 & 0.31 & 0.02 & 69.36 & 34.03 \\
         TrojNN & 1.0 & 0.99 & 9 & 53 & 0 & 8 & 0.0 & 0.01 & 0.0 & 0.02 & 68.14 & 35.34 \\
         Dynamic & 0.98 & 0.95 & 70 & 154 & 15 & 146 & 0.01 & 0.03 & 0.03 & 0.29 & 68.42 & 34.15 \\
         Reflection & 0.91 & 0.97 & 76 & 52 & 440 & 21 & 0.02 & 0.01 & 0.88 & 0.04 & 67.42 & 33.82 \\
         SIG & 0.97 & 0.99 & 100 & 43 & 52 & 7 & 0.02 & 0.01 & 0.1 & 0.01 & 67.61 & 34.47 \\
         Blend & 0.99 & 0.99 & 59 & 37 & 0 & 9 & 0.01 & 0.01 & 0.0 & 0.02 & 67.17 & 34.44 \\
         Invisible & 0.9 & 0.98 & 48 & 112 & 500 & 13 & 0.01 & 0.02 & 1.0 & 0.03 & 67.76 & 43.09 \\
         WaNet & 0.9 & 0.99 & 77 & 67 & 500 & 5 & 0.02 & 0.01 & 1.0 & 0.01 & 70.81 & 35.27 \\
         Gotham & 0.91 & 0.97 & 0 & 124 & 500 & 35 & 0.0 & 0.02 & 1.0 & 0.07 & 66.42 & 34.66 \\
         DFST & 0.91 & 0.91 & 0 & 83 & 500 & 404 & 0.0 & 0.02 & 1.0 & 0.81 & 68.0 & 35.53 \\
         \bottomrule
    \end{tabular}
    
    
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
         \toprule
         \multicolumn{13}{c}{\color[HTML]{FE0000} \textbf{GTSRB \& ResNet-18}} \\
         \midrule
         \textbf{Attack} & \multicolumn{2}{c}{\textbf{ACC}} & \multicolumn{2}{c}{\textbf{FP}} & \multicolumn{2}{c}{\textbf{FN}} & \multicolumn{2}{c}{\textbf{FFR}} & \multicolumn{2}{c}{\textbf{FAR}} & \multicolumn{2}{c}{\textbf{Time (s)}} \\
         \midrule
         BadNets & 0.94 & 1.0 & 0 & 0 & 336 & 0 & 0.0 & 0.0 & 0.67 & 0.0 & 144.7 & 35.01 \\
         TrojNN & 1.0 & 1.0 & 0 & 0 & 0 & 0 & 0.0 & 0.0 & 0.0 & 0.0 & 142.13 & 35.01 \\
         Dynamic & 0.99 & 1.0 & 0 & 9 & 61 & 1 & 0.0 & 0.0 & 0.12 & 0.0 & 141.6 & 33.78 \\
         Reflection & 0.91 & 0.99 & 0 & 5 & 500 & 47 & 0.0 & 0.0 & 1.0 & 0.09 & 141.66 & 33.74 \\
         SIG & 0.91 & 1.0 & 0 & 0 & 500 & 15 & 0.0 & 0.0 & 1.0 & 0.03 & 139.32 & 33.51 \\
         Blend & 0.93 & 1.0 & 0 & 0 & 371 & 0 & 0.0 & 0.0 & 0.74 & 0.0 & 142.94 & 32.93 \\
         Invisible & 0.91 & 1.0 & 0 & 1 & 500 & 0 & 0.0 & 0.0 & 1.0 & 0.0 & 142.78 & 48.46 \\
         WaNet & 0.91 & 1.0 & 0 & 0 & 500 & 0 & 0.0 & 0.0 & 1.0 & 0.0 & 149.2 & 33.97 \\
         Gotham & 0.93 & 1.0 & 0 & 0 & 372 & 7 & 0.0 & 0.0 & 0.74 & 1.0 & 141.5 & 33.22 \\
         DFST & 0.91 & 0.91 & 0 & 0 & 500 & 499 & 0.0 & 0.0 & 1.0 & 1.0 & 149.2 & 37.27 \\
         \bottomrule
    \end{tabular}

\end{table}

\iffalse
\begin{table*}[h]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=7pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Dataset Cleaning}
    \label{tab:data_clean}
    \begin{tabular}{c|cccccccccc}
         \toprule
         {\color[HTML]{FE0000} \textbf{CIFAR-10}} & \textbf{BadNets} & \textbf{TrojNN} & \textbf{Dynamic} & \textbf{Reflection} & \textbf{SIG} & \textbf{Blend} & \textbf{Invisible} & \textbf{WaNet} & \textbf{Gotham} & \textbf{DFST} \\
         \midrule
         ACC      & 0.98  & 0.99  & 0.95  & 0.97  & 0.99  & 0.99  & 0.98  & 0.99  & 0.97  & 0.91 \\
         FP       & 76    & 53    & 154   & 52    & 43    & 37    & 112   & 67    & 124   & 83 \\
         FN       & 9     & 8     & 146   & 21    & 7     & 9     & 13    & 5     & 35    & 404 \\
         FRR      & 0.02  & 0.01  & 0.03  & 0.01  & 0.01  & 0.01  & 0.02  & 0.01  & 0.02  & 0.02 \\
         FAR      & 0.02  & 0.02  & 0.29  & 0.04  & 0.01  & 0.02  & 0.03  & 0.01  & 0.07  & 0.81 \\
         Time (s) & 34.04 & 35.34 & 34.15 & 33.82 & 34.47 & 34.44 & 43.09 & 35.27 & 34.66 & 35.53 \\
         \bottomrule
    \end{tabular}
    
    \begin{tabular}{c|cccccccccc}
         \toprule
         {\color[HTML]{FE0000} \textbf{GTSRB}} & \textbf{BadNets} & \textbf{TrojNN} & \textbf{Dynamic} & \textbf{Reflection} & \textbf{SIG} & \textbf{Blend} & \textbf{Invisible} & \textbf{WaNet} & \textbf{Gotham} & \textbf{DFST} \\
         \midrule
         ACC & 1 & 1 & 0.99 & 0.99 & 1 & 1 &                             1 & 1 & 1 & 0.91 \\
         FP & 0 & 9 & 5 & 8 & 0 & 0 &                                    1 & 0 & 0 & 0 \\
         FN & 0 & 1 & 47 & 66 & 15 & 0 &                                 0 & 0 & 7 & 499 \\
         FRR & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 &                       0.0 & 0.0 & 0.0  & 0.0 \\
         FAR & 0.0 & 0.0 & 0.09 & 0.13 & 0.03 & 0.0 &                    0.0 & 0.0 & 0.01 & 1.0 \\
         Time (s) & 35.01 & 33.78 & 33.74 & 34.25 & 33.51 & 32.93 &      48.46 & 33.97 & 33.22 & 37.27 \\
         \bottomrule
    \end{tabular}

\end{table*}
\fi

==> tables/diff_dataset_effect.tex <==
\begin{table}[h]
    \centering
    % \footnotesize
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Inverted trigger effectiveness on different datasets/networks}
    \label{tab:diff_dataset_effect}
    \begin{tabular}{c|cc}
         \toprule
         \textbf{Attack} & \multicolumn{2}{c}{CIFAR-10/VGG-11 $\leftrightarrow$ GTSRB/ResNet18} \\
         \midrule
         BadNets & 1.0 & 1.0 \\
         TrojNN & 1.0 & 1.0 \\
         Dynamic & 1.0 & 1.0 \\
         Reflection & 0.95 & 0.84 \\
         Blend & 0.99 & 1.0 \\
         SIG & 0.90 & 0.86 \\
         Invisible & 0.96 & 0.89 \\
         WaNet & 0.80 & 0.73 \\
         Gotham & 0.95 & 0.99 \\
         DFST & 0.81 & 0.87 \\
         \bottomrule
    \end{tabular}
\end{table}


==> tables/forensic_time.tex <==
& Time (min)
& 87.8  & 83.1 & 98.3 & 95.2 & 98.8
& 67.2 & 57.5 & 53.8 & 53.6 & 54.4
& 28.7 & 27.5 & 28.0 & 28.4 & 31.6 & 28.4 & 32.9 & 27.7 & 30.9 & 29.6 & 35.2
& 32.6 & 32.2 & 30.0 & 35.9 & 30.4 & 36.4 & 31.7 & 33.6 & 31.7 & 37.0 & 32.2
Average: 45.1 minutes

% mask, trigger, linear, average

==> tables/model_checking.tex <==
\begin{table*}[h]
    \centering
    % \footnotesize
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=7pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Model Checking (100 random images)}
    \label{tab:model_check}
    \begin{tabular}{c|cccccccccc}
         \toprule
         {\color[HTML]{FE0000} \textbf{CIFAR-10}} & \textbf{BadNets} & \textbf{TrojNN} & \textbf{Dynamic} & \textbf{Reflection} & \textbf{SIG} & \textbf{Blend} & \textbf{Invisible} & \textbf{WaNet} & \textbf{Gotham} & \textbf{DFST} \\
         \midrule
         ACC & 0.87 $\pm$ 0.02 & 0.86 $\pm$ 0.04 & 0.87 $\pm$ 0.02 & 0.87 $\pm$ 0.02 & 0.86 $\pm$ 0.02 & 0.87 $\pm$ 0.02 & 0.86 $\pm$ 0.03 & 0.89 $\pm$ 0.03 & 0.86 $\pm$ 0.02 & 0.86 $\pm$ 0.01 \\
         ASR & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.01 & 0.99 $\pm$ 0.01 & 0.99 $\pm$ 0.01 & 1.0 $\pm$ 0.0 & 0.99 $\pm$ 0.01 & 0.98 $\pm$ 0.02 & 1.0 $\pm$ 0.01 & 0.99 $\pm$ 0.01 \\
         \hline
         PN-ASR & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 0.97 $\pm$ 0.05 & 0.98 $\pm$ 0.04 & 0.6 $\pm$ 0.25 & 0.8 $\pm$ 0.15 & 0.97 $\pm$ 0.05 & 0.67 $\pm$ 0.18 \\
         CN-ASR & 0.18 $\pm$ 0.08 & 0.31 $\pm$ 0.09 & 0.26 $\pm$ 0.05 & 0.47 $\pm$ 0.12 & 0.3 $\pm$ 0.1 & 0.41 $\pm$ 0.17 & 0.23 $\pm$ 0.07 & 0.18 $\pm$ 0.04 & 0.27 $\pm$ 0.08 & 0.24 $\pm$ 0.07 \\
         \hline
         CK-ACC & 1.0 & 1.0 & 1.0 & 0.9 & 1.0 & 0.95 & 0.8 & 1.0 & 1.0 & 0.85 \\
         FP & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
         FN & 0 & 0 & 0 & 0 & 0 & 0 & 4 & 0 & 0 & 3 \\
         \hline
         Time (s) & 7.4 & 7.0 & 7.7 & 8.1 & 7.4 & 5.9 & 7.6 & 7.6 & 7.59 & 8.7 \\
         \bottomrule
    \end{tabular}
    
    \begin{tabular}{c|cccccccccc}
         \toprule
         {\color[HTML]{FE0000} \textbf{GTSRB}} & \textbf{BadNets} & \textbf{TrojNN} & \textbf{Dynamic} & \textbf{Reflection} & \textbf{SIG} & \textbf{Blend} & \textbf{Invisible} & \textbf{WaNet} & \textbf{Gotham} & \textbf{DFST} \\
         \midrule
         ACC & 0.94 $\pm$ 0.02 & 0.94 $\pm$ 0.01 & 0.94 $\pm$ 0.01 & 0.94 $\pm$ 0.03 & 0.93 $\pm$ 0.04 & 0.94 $\pm$ 0.02 & 0.93 $\pm$ 0.02 & 0.92 $\pm$ 0.05 & 0.94 $\pm$ 0.01 & 0.94 $\pm$ 0.01 \\
         ASR & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 0.87 $\pm$ 0.06 & 0.83 $\pm$ 0.1 & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 0.98 $\pm$ 0.02 & 1.0 $\pm$ 0.0 & 0.99 $\pm$ 0.01 \\
         \hline
         PN-ASR & 1.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 0.99 $\pm$ 0.03 & 0.85 $\pm$ 0.09 & 0.81 $\pm$ 0.11 & 1.0 $\pm$ 0.0 & 0.45 $\pm$ 0.14 & 0.59 $\pm$ 0.22 & 1.0 $\pm$ 0.0 & 0.82 $\pm$ 0.15 \\
         CN-ASR & 0.17 $\pm$ 0.08 & 0.33 $\pm$ 0.08 & 0.17 $\pm$ 0.07 & 0.38 $\pm$ 0.13 & 0.31 $\pm$ 0.14 & 0.24 $\pm$ 0.08 & 0.18 $\pm$ 0.04 & 0.16 $\pm$ 0.08 & 0.25 $\pm$ 0.08 & 0.22 $\pm$ 0.06 \\
         \hline
         CK-ACC & 1.0 & 1.0 & 1.0 & 0.9 & 1.0 & 1.0 & 0.65 & 0.75 & 1.0 & 0.95 \\
         FP & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
         FN & 0 & 0 & 0 & 0 & 0 & 0 & 7 & 5 & 0 & 1 \\
         \hline
         Time (s) & 8.3 & 8.5 & 8.1 & 7.6 & 5.6 & 8.0 & 8.4 & 7.8 & 7.9 & 6.8 \\
         \bottomrule
    \end{tabular}

\end{table*}


==> tables/trigger_type_recog.tex <==
\begin{table*}[H]
    \centering
    \footnotesize
    \tabcolsep=5pt
    \caption{Summarization for Different Attacks}
    \begin{tabular}{cccccccc}
        \toprule
         Attack & BadNets & Dynamic & Reflection & SIG & Invisible & WaNet & Gotham \\
         \toprule
         Cluster & Binomial & Binomial & Constant & Constant & Complex & Complex & Simple \\
         \midrule
         Accuracy & 1.00 & 1.00 & 0.98 & 0.94 & 0.97 & 0.91 & 1.00 \\
         \bottomrule
    \end{tabular}
    \label{tab:trigger_type}
\end{table*}


==> tables/trojai_eval_v0.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=6pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Evaluation on TrojAI}
    \label{tab:eval_trojai}
    \begin{tabular}{c|ccc|ccc}
         \toprule
         % change to multirow{2}
         \multirow{3}{*}{\textbf{Technique}} & \multicolumn{6}{c}{\textbf{Polygon}} \\
         ~ & \multicolumn{3}{c}{\textbf{Round 2 (552 Clean + 276 Poison)}} & \multicolumn{3}{c}{\textbf{Round 3 (504 Clean + 251 Poison)}} \\
         ~ & FP & FN & ACC & FP & FN & ACC \\
         \midrule
         K-arm (Random\_Init) & 10 & 178 & 0.773 & 7 & 107 & 0.849 \\
         K-arm (Central\_Square) & 21 & 94 & 0.861 & 13 & 49 & 0.918 \\
         K-arm (Forensic) & 19 & 85 & \textbf{0.874} & 10 & 50 & \textbf{0.921} \\
         \hline\hline
         ABS (Random\_Init) & ? & ? & ? & 92 & 100 & 0.746 \\
         ABS (Random\_Square) & ? & ? & ? & 22 & 49 & 0.906 \\
         ABS (Topleft\_Square) & ? & ? & ? & 16 & 86 & 0.865 \\
         ABS (Central\_Square) & ? & ? & ? & 30 & 38 & 0.910 \\
         ABS (Forensic) & 67 & 34 & 0.878 & 23 & 33 & \textbf{0.926} \\
         \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[h]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.2}
    \tabcolsep=7pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Evaluation on TrojAI}
    \label{tab:eval_trojai}
    \begin{tabular}{c|ccc|ccc}
         \toprule
         % change to multirow{2}
         \multirow{3}{*}{\textbf{Technique}} & \multicolumn{6}{c}{\textbf{Instagram Filter}} \\
         ~ & \multicolumn{3}{c}{\textbf{Round 2 (552 Clean + 276 Poison)}} & \multicolumn{3}{c}{\textbf{Round 3 (504 Clean + 252 Poison)}} \\
         ~ & FP & FN & ACC & FP & FN & ACC \\
         \midrule
         Direclt\_Apply & ? & ? & ? & 179 & 5 & 0.757 \\
         Partial\_Apply & ? & ? & ? & 89 & 14 & 0.864 \\
         ABS (Pooling) & 25 & 98 & 0.851 & 34 & 109 & 0.811 \\
         ABS (Forensic) & 28 & 34 & \textbf{0.912} & 8 & 67 & \textbf{0.901} \\
         \bottomrule
    \end{tabular}
\end{table*}
